Training LayoutLM from Scratch for Efficient Named-Entity Recognition in the Insurance Domain

Generic pre-trained neural networks may struggle to produce good results in specialized domains like finance and insurance. This is due to a domain mismatch between training data and downstream tasks, as in-domain data are often scarce due to privacy constraints. In this work, we compare different pre-training strategies for LayoutLM. We show that using domain-relevant documents improves results on a named-entity recognition (NER) problem using a novel dataset of anonymized insurance-related financial documents called Payslips. Moreover, we show that we can achieve competitive results using a smaller and faster model.

==> tables/datasets.tex <==

\begin{table*}
\centering
\small
\begin{tabular}{lccll}
\toprule
 \textbf{Dataset} & \makecell{\textbf{Train / Val / Test size} \\ (\# pages)} & \makecell{\textbf{\% of O} \\ (word level)} &\textbf{Document Type} &\textbf{Main entity types}  
\\
\midrule
\textsc{FUNSD} \cite{jaume2019funsd} & $149$ / - / $50$ & $0 $ &Forms&Text   
\\
\textsc{SROIE} \cite{SROIE_Huang_2019} & $626$  / - /  $347$ & $83.82$ &Receipts &Text, Dates, Amounts 
\\
\textsc{CORD} \cite{park2019cord} & $800$  / $100$ / $100$ & $0$ &Receipts &Text, Dates, Amounts 
\\
\textsc{DOCILE} labeled \cite{simsa_docile_2023} & $6,759$ / $635$ / $1,000$ & $89.46$ &Invoices &Text, Dates, Amounts  
\\
\textsc{Payslips} (ours)& $485$ / - / $126$ & $95.30$ &Pay Statements &Dates, Amounts \\
\bottomrule
\end{tabular}
\caption{Overview of annotated datasets for Named Entity Recognition (NER) in documents. The percentage of \textsc{O} labels is calculated based on the combined train, validation and test sets, except for \textsc{DOCILE} labeled, where test annotations are unavailable, and the percentage is based on the train and validation sets.}
\label{tab:datasets}
\end{table*}
